Data-CASE: Grounding Data Regulations for Compliant Data Processing Systems

Data regulations, such as GDPR, are increasingly being adopted globally to protect against unsafe data management practices. Such regulations are, often ambiguous (with multiple valid interpretations) when it comes to defining the expected dynamic behavior of data processing systems. This paper argues that it is possible to represent regulations such as GDPR formally as invariants using a (small set of) data processing concepts that capture system behavior. When such concepts are grounded, i.e., they are provided with a single unambiguous interpretation, systems can achieve compliance by demonstrating that the system-actions they implement maintain the invariants (representing the regulations). To illustrate our vision, we propose Data-CASE, a simple yet powerful model that (a) captures key data processing concepts (b) a set of invariants that describe regulations in terms of these concepts. We further illustrate the concept of grounding using "deletion" as an example and highlight several ways in which end-users, companies, and software designers/engineers can use Data-CASE.

==> fig/graph_controller_delete.tex <==
\begin{tikzpicture}
\begin{axis} [name = plot1, height=4.5cm,
        width=7.5cm,
        %x tick label style={xshift=0.4cm},
        %xmin=-1,
        ymin=0,
        ymax=16000,
        xmin = 0,
        xmax = 11,
        xticklabel shift= 0in,
        xtick={1,4,7, 10},
        xtick pos=bottom,
        % xlabel shift=2in,
        %every access x label/.style={at=(ticklabel cs: 2,0)}, anchor=north,
        xticklabels = {10K, 30K, 50K, 70K},
        x tick label style = {font = \tiny, rotate=0},
        y tick label style = {font = \tiny, rotate=0},
        ylabel=Time to run WCon (seconds),
        xlabel= {Number of Transactions},
        x label style = {font=\small},
        y label style = {font=\small},
        legend style={
          at={(0,1)},
          anchor=north west, font =\small, legend columns = 1, draw=none, fill = none
        },
        % nodes near coords,
        % every node near coord/.append style={font=\tiny},
        ybar=0pt, %ybar=0pt means bar stick together
        bar width=6pt,
        legend pos= north west,
        legend style={legend cell align=left, font=\tiny, legend columns=1},
        %bottom line makes single bar appear in legend
        legend image code/.code={\draw [#1] (0cm, -0.1cm) rectangle (0.2cm, 0.125cm);},
        ytick = {0, 1000, 2000, 3000, 4000, 8000, 12000, 16000},
        ymajorgrids, yminorgrids,
]
\addplot [fill=teal]  coordinates {(1,376) (4,1003) (7,1472) (10,1966)};
\addlegendentry {DELETE + VACUUM}
\addplot [pattern=horizontal lines, pattern color=red] coordinates {(1,412) (4,1044) (7,1617) (10,2042)};
\addlegendentry {DELETE}
\addplot [pattern=north east lines, pattern color=brown] coordinates {(1,459) (4,1321) (7,2261) (10,3247)};
\addlegendentry {Tombstones (Indexing)}
\addplot [pattern=north west lines, pattern color=black]coordinates {(1,2391) (4,7106) (7,11248) (10,14826)};
\addlegendentry {DELETE and VACUUM FULL}
\end{axis}
\end{tikzpicture}
